Strategic Defense against Stealthy Link Flooding Attacks: A Signaling Game Approach

With the increasing diversity of Distributed Denial-of-Service (DDoS) attacks, it is becoming extremely challenging to design a fully protected network. For instance, Stealthy Link Flooding Attack (SLFA) is a variant of DDoS attacks that strives to block access to a target area by flooding a small set of links, and it is shown that it can bypass traditional DDoS defense mechanisms. One potential solution to tackle such SLFAs is to apply Moving Target Defense (MTD) techniques in which network settings are dynamically changed to confuse/deceive attackers, thus making it highly expensive to launch a successful attack. However, since MTD comes with some overhead to the network, to find the best strategy (i.e., when and/or to what extent) of applying it has been a major challenge. The strategy is significantly influenced by the attacker's behavior that is often difficult to guess. In this work, we address the challenge of obtaining the optimal MTD strategy that effectively mitigates SLFAs while incurs a minimal overhead. We design the problem as a signaling game considering the network defender and the attacker as players. A belief function is established throughout the engagement of the attacker and the defender during this SLFA campaign, which is utilized to pick the best response/action for each player. We analyze the game model and derive a defense mechanism based on the equilibria of the game. We evaluate the technique on a Mininet-based network environment where an attacker is performing SLFAs and a defender applies MTD based on equilibria of the game. The results show that our signaling game-based dynamic defense mechanism can provide a similar level of protection against SLFAs like the extensive MTD solution, however, causing a significantly reduced overhead.

==> table.tex <==

\begin {table}[h]
\begin{center}
\caption {Packet Loss Percentage Caused by Flow Table Update} \label{tab:switchingcost} 
  \begin{tabular}{ | c |  c | c | c |}
    \hline
      10-sec RRM & 30-sec RRM & 60-sec RRM & 120-sec RRM  \\ \hline
    10.1  &   8.6 \%  & 1.6\% & 0.5\%  \\ \hline %17.3
  \end{tabular}
\end{center}
\end {table}



%update table:
%120rrm (15257)
%3724-3058-4242-4243  
%10rrm (16195)
%3853-3235-4815-4295

%60rrm (15057)
%3925-4769-2927-3436
%4202-4554-3084-3619 (15459)
%300rrm
%12888

%Abdullah Aydeger, Mohammad Hossein Manshaei, Mohammad Ashiqur Rahman, and Kemal Akkaya


\subsubsection{Dynamic Belief}

In addition to the initial belief, we define the dynamic belief function that will be calculated at each time the game is played. We consider three different factors that can have an impact on the dynamic belief. The highest impact is the previous belief of the current bot (i.e., $\theta_j(i-1)$). We take this into consideration and assign the weight value as 90\% of the total belief function \remark{Why is 90\%? We should not take these values directly. Use variables while we can have example values with some justifications.}
%since each client is supposed to be responsible for his/her own history. The reason is 
. The main reason is that if a client has been behaving suspicious for most of the time previously, it is highly possible he is one of the bots being used by attacker. This metric is based on some learning processes throughout the time. Second one is the belief for the rest of the network nodes (i.e., $\sum_{k=0}^{Nr}  \theta_k(i-1)$), since it is DDoS attack and it is performed by multiple bots. Last metric we use to update our belief is the last packet we received from the specific bot (i.e., $A(i)$). Even though it has very small impact (i.e., 1\%) by itself, it adds up rapidly if the bot continuously takes malicious actions.
Hence, this belief for $j^{th}$ client at time $i$ is calculated by,

\begin{equation}
\label{Eq:belief}
\theta_j(i) = \theta_j(i-1) \times 0.9 + \frac {\sum_{k=0}^{Nr}  \theta_k(i-1)} {i-1} \times 0.09 +  A(i) \times 0.01
\end{equation}



\begin {table}[h]
\begin{center}
\caption {Packet Loss} \label{tab:attackercost} 
  \begin{tabular}{ | l |  c |  c | c | c |}
    \hline
     Client  &  \multicolumn{4}{|c|}{Packet Loss} \\
     \cline{2-5}
      ID &No Defense &  10-sec RRM & 30-sec RRM & 60-sec RRM\\ \hline
    1  &   18.2\%  & 4.2\% & 7.8\% & 6.8\% \\ \hline %17.3
    2  &   15.2\%  & 3.1\% & 2.4\% & 5.1\% \\ \hline %14.4
    3  &   0       & 5\%   & 3\%   & 4.1\% \\ \hline 
    4  &   0       & 1.9\% & 6.7\% & 3.7\% \\ \hline 
Overall&   8.3\%   & 3.5   & 5\%   & 5\%   \\ \hline %8.1
  \end{tabular}
\end{center}
\end {table}




\begin{figure}
\centering
\includegraphics[width=3.6in]{figures/switching-delay-rrm.pdf}%\vspace{-0.5em}
\caption{Switching Delay in Different Periods of RRM}
\label{fig:rrmcomparison}
\end{figure}


\begin {table*}[h]
\begin{center}
\caption {Delay Caused by RRM (in Microsecond)} \label{tab:delayrrm} 
  \begin{tabular}{ | c | c |  c |  c |  c | c |  c | }
    \hline
     \textbf{\textit{Delay }} & 
     \multicolumn{6}{|c|}{\textbf{\textit{Delay with RRM}}}  \\
     \cline{2-7}
     \textbf{\textit{Without  }} & 
     \multicolumn{3}{|c|}{\textbf{\textit{Same size Path}}} & 
     \multicolumn{3}{|c|}{\textbf{\textit{Any size Path}}}  \\
     \cline{2-7}
     \textbf{\textit{RRM}} &\textit{\textbf{60-sec RRM}} & \textit{\textbf{30-sec RRM}} & \textit{\textbf{10-sec RRM}} & \textit{\textbf{60-sec RRM}} & \textit{\textbf{30-sec RRM}} & \textit{\textbf{10-sec RRM}}\\
     \cline{1-2}
     \hline 
   %  & Optimum Delay &  (same size paths only) & Delay with RRM (\\ \hline
   % id - norrm - rrm10sec2path - rrm10secany
     2175 & 2371 & 2510 & 2846 & 3125 & 3153 & 3531 \\ \hline 
  \end{tabular}
\end{center}
\end{table*}















	\begin{table*}[t]
		\centering
		\caption{Equilibria and Their Conditions \remark{Yet to apply the comments}}
		\label{Table_PBNE}
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			\multirow{2}{*}{Theorem}&
			\multirow{2}{*}{Conditions}&\multirow{2}{*}{Range of $\theta$} & \multirow{2}{*}{$\#$}& \multirow{2}{*}{$PBNE$}& \multicolumn{2}{|c|}{Condition on Beliefs}\\
			\cline{5-6}
			%            Scenario & First player strategy & second player strategy & On-equilibrium path's beliefs  & Off-equilibrium path's beliefs & condition on $\theta$ & Others condition\\
			&ٍ  && &On-equilibrium & Off-equilibrium\\
			\hline
			%    \rowcolor{gray}{30!}
			Theorem 1& \multirow{2}{*}{$-$}&$\theta\ge\theta^{*}$& $\mathcal{PBNE}_{1}$ & $\{(N,N),(R,\overline{R}),p,q\}$ &$p=\theta$ & $ \forall q$\\
				Theorem 2&\cline{2-6 }
			&$\theta\le\theta^{*}$ &$\mathcal{PBNE}_{2}$ & $\{(N,N),(\overline{R},\overline{R},),p,q\}$ &$p=\theta$ & $ \forall q$\\
%			\hline    
%			$c_{nl}^{m}\le c_{l}^{m}\le c_{nl}^{m}+\epsilon$&$-$&$-$&$-$&$-$&$-$\\
			\hline
			Theorem 2&$\lambda \ge\lambda^* $&$\forall \theta^{*}$&$\mathcal{PBNE}_{3}$&$\{(N,G),(R,\overline{R}),p,q\}$&$p=1$&$q=0$\\
			\hline 
		Theorem 2&$\lambda \le\lambda^* $&$\forall \theta^{*}$&$\mathcal{PBNE}_{4}$&$\{(N,G),(\overline{R},\overline{R}),p,q\}$&$p=1$&$q=0$\\
			\hline 
			
		\end{tabular}
	\end{table*}

powerfulaggressive - stealth - decentaggr- st
str: 198317 -119540 - 26119 - 13584 
rrm: 267375- 85394 - 21791 - 8494
norrm: 376102 - 182209 - 90658 - 41011


438  - 278  -  200   - 141
989  - 280  -  251   -  168
1172 - 579  - 464    -   263


-141
-68



rrm 133



\subsubsection{Analyzing Periodic RRM with the Attacker}

Here, we execute experiments considering an attacker and observe the impact of the attack at different frequencies of RRM. 
The attacker is aggressive with decent capabilities. 
As shown in Table \ref{tab:attackercost}, there is an average of 8.3\% overall packet loss in the network, if there is \textit{No Defense} running. If we apply RRM %at every few seconds (10, 30, or 60 seconds) 
we get more balanced traffic and less overall packet loss in the network. Even though 10-second RRM gives the best results, i.e., 3.5\% packet loss on average while defending against the Crossfire attack as can be seen in Table \ref{tab:attackercost} \remark{Justification?}, 60-second RRM causes less delays and less packet loss if there is no attack, as shown in Tables~\ref{tab:delayrrm} and~\ref{tab:switchingcost}. 
In other words, if there is no attack, 10-second RRM causes lots of overhead compared to 60-second RRM. Thus, we opt to run 60-second RRM in our following experiments to compare with \textit{Strategic RRM}. %Remember that, this configuration may change according to the network %Remember that, RRM may affect all clients in the network. We compare our strategic RRM based defense mechanism with 60-sec RRM based mechanism in the following experiments.

\begin {table}[t]
\begin{center}
\caption {Packet Loss} \label{tab:attackercost} 
  \begin{tabular}{ | l |  c |  c | c | c |}
    \hline
     Client  &  \multicolumn{4}{|c|}{Packet Loss} \\
     \cline{2-5}
      ID &No Defense &  10-sec RRM & 30-sec RRM & 60-sec RRM\\ \hline
    1  &   18.2\%  & 4.2\% & 7.8\% & 6.8\% \\ \hline %17.3
    2  &   15.2\%  & 3.1\% & 2.4\% & 5.1\% \\ \hline %14.4
    3  &   0       & 5\%   & 3\%   & 4.1\% \\ \hline 
    4  &   0       & 1.9\% & 6.7\% & 3.7\% \\ \hline 
Overall&   8.3\%   & 3.5   & 5\%   & 5\%   \\ \hline %8.1
  \end{tabular}
\end{center}
\end {table}

==> threat.tex <==
\subsection{Adversary Model}
In this paper, we use Crossfire attack as our threat. Our model is implemented and configured based on the given attack definition in Section \ref{sec:crossfire}. Two different approaches are considered for attacker, namely stealthy and aggressive. Stealthy attacker is not in rush to conduct the attack. He takes his time to run reconnaissance attack and creates target link set accordingly. He also stays idle sometimes in order to behave like legitimate users. After that he starts data phase of attack to exhaust the links' bandwidth. Meanwhile, aggressive attacker behaves more greedy and transmits more quickly to congest links. Reconnaissance attack is performed in given short time. The information is collected and the attack pattern is designed within this time.

Furthermore, attacker is assumed to have limited number of bots. Thus, two different capabilities are considered for an adversary; decent, and powerful. For decent adversary model, we consider the number of bots that attacker is able to manipulate is as many as legitimate clients in the network. We extend attacker's capabilities and double the number of bots for powerful adversary model.


%namely lightweight, reasonable, and greedy. 



%In our paper, we use Crossfire attack as our threat. Our model is implemented and configured based on the given attack definition in Section \ref{sec:crossfire}. Attacker's reconnaissance time is set to 10 seconds and data phase of the attack as 1 minute. After data phase is conducted, new reconnaissance attack will be run in order to detect new target link set if any of the routes is changed. These processes are continued throughout the game. Bot master manages different bots in different locations in the network. Each bot is configured to transfer maximum of 5 Mbps data traffic to the decoy servers. Bot master is the one playing the game with defender (network admin). He selects which bots to send data at each time he creates the target link set. 

%We assume that the number of bots that Bot Master can have is restricted that Bot Master is not able to congest all network links. In other words, Bot Master is only capable of having two links as the target link set. 

